In-Network View Synthesis for Interactive Multiview Video Systems

To enable Interactive multiview video systems with a minimum view-switching delay, multiple camera views are sent to the users, which are used as reference images to synthesize additional virtual views via depth-image-based rendering. In practice, bandwidth constraints may however restrict the number of reference views sent to clients per time unit, which may in turn limit the quality of the synthesized viewpoints. We argue that the reference view selection should ideally be performed close to the users, and we study the problem of in-network reference view synthesis such that the navigation quality is maximized at the clients. We consider a distributed cloud network architecture where data stored in a main cloud is delivered to end users with the help of cloudlets, i.e., resource-rich proxies close to the users. In order to satisfy last-hop bandwidth constraints from the cloudlet to the users, a cloudlet re-samples viewpoints of the 3D scene into a discrete set of views (combination of received camera views and virtual views synthesized) to be used as reference for the synthesis of additional virtual views at the client. This in-network synthesis leads to better viewpoint sampling given a bandwidth constraint compared to simple selection of camera views, but it may however carry a distortion penalty in the cloudlet-synthesized reference views. We therefore cast a new reference view selection problem where the best subset of views is defined as the one minimizing the distortion over a view navigation window defined by the user under some transmission bandwidth constraints. We show that the view selection problem is NP-hard, and propose an effective polynomial time algorithm using dynamic programming to solve the optimization problem. Simulation results finally confirm the performance gain offered by virtual view synthesis in the network.

==> DP_solution.tex <==
 
 
 
 
 \begin{figure}[t]
\subfigure[]{
 \includegraphics[width=0.45\linewidth ,draft=false]{figure/Distorted_Region_B_3.eps} 
 \label{fig:Distorted_B}
 }
 \hfil
 \subfigure[]{
 \includegraphics[width=0.45\linewidth ,draft=false]{figure/Distorted_Region_C.eps} 
 \label{fig:Distorted_C}
 }
 \hfil
 \subfigure[]{
 \includegraphics[width=0.45\linewidth ,draft=false]{figure/Distorted_Region_D.eps} 
 \label{fig:Distorted_D}
 }
 \hfil \caption{Covering regions in the case of undistorted views.  Case (b) contradicts the independence of optimality for left and right reference view. Cases (c) and (d) are feasible solutions under both assumptions.}\label{fig:Distorted_Region}
 \end{figure}
%
   
Optimization in \eqref{eq:optimization} selects a pair of reference views for each virtual view in the navigation window. We can graphically illustrate the selected reference views for virtual views in the window as shown in Fig.\;\ref{fig:Distorted_A}. In the figure, the $x$-axis represents the virtual views in the navigation window $[U_L^0, U_R^0]$ that require synthesis. Correspondingly, the $y$-axis represents the reference views selected for synthesis of each virtual view $u$ in the navigation window; \textit{i.e.}, for each $u \in [U_L^0, U_R^0]$, there must either be selected reference pair $(v_L, v_R)$ such that $v_L < u < v_R$, or there is a selected reference $v = u$, in which case $v$ can be used directly as virtual view $u$ with no view synthesis. A horizontal line segment---\textit{e.g.}, $v=v_1$ for $U^0_L \leq u \leq v_3$ in Fig.\;\ref{fig:Distorted_A}---means the same reference is used for a range of virtual views. As shown, this graphical representation results in two step functions above and below the $u=v$ line, representing the selected right and left reference views respectively. The set of selected reference views are the union of the distinct step locations of the two step functions. 

%A black solid line for $v_i$ for all viewpoints in the range $[u_L,u_R]$ means that view $v_i$ is selected as reference view for that range.   Fig. \ref{fig:Distorted_Region} depicts the feasible solution spaces for  distorted reference views. In particular, for each $u$, one left and right reference view is selected above and below the $u=v$ line respectively. This satisfies the condition $V_L\leq u \leq V_R$. However, no other constraints are imposed. For example, the closest reference view might not be the optimal one for virtually synthesizing a viewpoint. This usually happens if the closest reference view  is much more distorted than a more far a part reference view.  Among all cases depicted in  Fig. \ref{fig:Distorted_Region}, we are interested in understanding which are the feasible scenarios under the distortion assumptions discussed in Sec. \ref{sec:sub:View_Distortion}.


This graphical representation of selected references is very useful in visualizing different kinds of solutions to \eqref{eq:optimization}. For example, under the assumption of shared reference optimality as discussed in Section \ref{sec:sub:View_Distortion}, we see that the selected reference views in Fig.\;\ref{fig:Distorted_A} cannot be an optimal solution. Specifically, virtual views $v_3 - 1/L$ and $v_3 + 1/L$ employ references $[v_1, v_4]$ and $[v_2, v_5]$ respectively.  However, if references $[v_1, v_4]$ are better than $[v_2, v_5]$ for virtual view $v_3 - 1/L$, they should be better for virtual view $v_3 + 1/L$ also according to shared reference optimality in \eqref{eq:shared_optimality}.



==> NPproof.tex <==
\label{eq:np_hard_proof}
 \begin{figure}[t]
 \begin{center}
 \includegraphics[width=0.4\linewidth ,draft=false]{figure/NP_Hardness.eps} 
 \caption{Example of items set $\mathcal{S}$ and collection of sets  $\mathcal{C}$, with $|\mathcal{S}|= 5$ and $|\mathcal{C}|= 4$.}\label{fig:NP_Hardness}
 \end{center}
 \end{figure}

We now outline a proof-by-construction that shows the reference view selection problem (\ref{eq:optimization}) is NP-hard by reducing the known NP-hard \textit{set cover} (SC) problem to a special case of the reference view selection problem. In SC, a set of items $\mathcal{S}$ (called the universe) are given, together with a defined collection $\mathcal{C}$ of subsets of items  in $\mathcal{S}$. The SC problem is to identify at most $K$ subsets from collection $\mathcal{C}$ that covers $\mathcal{S}$, \textit{i.e.}, a smaller collection $\mathcal{C}^{\prime}\subseteq  \mathcal{C} $ with $|\mathcal{C}^{\prime}| \leq K$ such that every item in $\mathcal{S}$ belongs to at least one subset in collection $\mathcal{C}^{\prime}$. 

We construct a corresponding special case of our reference view selection problem as follows. For each item $i$ in $\mathcal{S} = \{1, \ldots, |\mathcal{S}|\}$ in the SC problem, we first construct an undistorted reference view $i$. In addition, we construct a default undistorted right reference view $|\mathcal{S}|+1$, and the navigation window is set to $[U^0_L, U^0_R] = [1, |\mathcal{S}|+1]$ and $L=2$. Further, for each item $i$ in $\mathcal{S}$, we construct a virtual view $i + \frac{1}{2}$ that requires the selection of left reference $i$, in combination of default right reference $|\mathcal{S}|+1$, for the resulting synthesized view distortion $d_{i + \frac{1}{2}}(i,|\mathcal{S}|+1,0,0)$ to achieve distortion $\bar{D} < \infty$. Thus the selection of $|\mathcal{S}|$ left references and one default right reference $|\mathcal{S}|+1$ consumes $|\mathcal{S}|+1$ views worth of bandwidth already. See Fig.~\ref{eq:np_hard_proof} for an illustration. Note that given this selection of left reference views, any selection of right reference views will satisfy the shared optimality of reference views assumption. 

For each subset $j$ in collection $\mathcal{C} = \{1, \ldots, |\mathcal{C}|\}$ in the SC problem, we construct a right reference view $|\mathcal{S}| + 1 + j$, such that if item $i$ belongs to subset $j$ in the SC problem, the synthesized distortion $d_{i + \frac{1}{2}}(i,|\mathcal{S}|+1+j,0,0)$ at virtual view $1 + \frac{1}{2}$ will be reduced to $\bar{D} - \Delta$ given right reference view $|\mathcal{S}| + 1 + j$ is used. The corresponding binary decision we ask is: given channel bandwidth of $|\mathcal{S}| + 1 + K$, is there a reference view selection such that the resulting synthesized view distortion is $|\mathcal{S}| (\bar{D} - \Delta)$ or less?

From construction, it is clear that to minimize overall distortion, left reference views $1, \ldots, |\mathcal{S}|$ and default right reference view $|\mathcal{S}| + 1$ must be first selected in any solution with distortion $< \infty$. Given remaining budget of $K$ additional views, if distortion of $|\mathcal{S}| (\bar{D} - \Delta)$ is achieved, that means $K$ or fewer additional right reference views are selected to reduce synthesized distortion from $\bar{D}$ to $\bar{D} - \Delta$ at each of the virtual view $i + \frac{1}{2}$, $i \in \{1, \ldots, |\mathcal{S}|\}$. Thus these additionally $K$ or fewer selected right reference views correspond exactly to the subsets in the SC problem that covers all items in the set $\mathcal{S}$. This solving this special case of the reference view selection problem is no easier than solving the SC problem, and therefore the reference view selection problem is also NP-hard. $\Box$


%In particular, for each  $v_i \in \mathcal{S}$ we identify a range of viewpoints that will be virtually synthesized with  $v_i$ as right view. The union of these ranges associated to all $v_i$'s  in $\mathcal{S}$ equals $[U_L^0, U_R^0]$.  Let $\mathcal{C}$ be the set of $|\mathcal{C}|$ possible right reference views greater than $U_R^0$. Let also denote by $v_R$ the default reference view (greater than any right view in $\mathcal{C}$).  For each left view $v_j$ in the subset $\mathcal{C}^{\prime}$, a portion of   viewpoint ranges will adopt  $v_j$ as right reference view (i.e.,   all the ranges in which $v_j$ is the best right reference view) while the remaining ones will adopt the default right reference view $v_R$ as right view. The distortion gain in using $v_j$ as right reference view  rather than $v_R$ is   of $\Delta$ for each range adopting $v_j$, and $0$ otherwise.  In the example in Fig. \ref{fig:NP_Hardness}, we have that the subset $\mathcal{C}^{\prime}$ can cover the ranges $[v_2,v_3]$ and $[v_3,v_4]$ that can be virtually synthesized at a distortion  lower than the one experienced with the default right reference view.  The experienced distortion is of $\Delta$ for both ranges. 


%Finally, let the maximum number of reference views to select be $C = |\mathcal{S}| +K +1$. If an optimal solution of  the optimization problem in Eq. \eqref{eq:optimization} has  $|\mathcal{S}|$ left reference views and $K+1$ right views and if the solution is  such that the distortion of the virtually synthesized viewpoints in $[U_L^0,U_R^0]$ has an improvement of   $ |\mathcal{S}| \Delta$ w.r.t. the case in which the default right view is adopted over the entire range, than the selected right camera views will correspond to  $\mathcal{C}^{\prime}$ in \ac{SC}. Hence, \ac{SC} is a special case of the problem optimization in Eq. \eqref{eq:optimal_1}. 



==> algo.tex <==
It is clear that the reference view selection problem in \eqref{eq:optimization} in its most general form when no assumptions are made on the synthesized view distortion function $d_u(\,)$ is NP-hard. In fact, even with the shared reference optimality assumption, the problem remains NP-hard. Sketch of an NP-hardness proof is provided in Appendix \ref{sec:appendix_C}. Nonetheless, with the shared reference optimality assumption, we can construct a tractable exponential time algorithm that yields an optimal solution. We develop this algorithm in this section.

\subsection{Algorithm}

Let consider the $i$-th optimization step ($i>1$), in which the first $C-k$ reference views has been already selected, and the remaining $k$ has to be discovered.  At this step, $v_i>v_{i-1}$ has to be optimized, where $v_{i-1}$ is the reference views selected at the $(i-1)$-th optimization step. 
We denote by $\mathcal{L}: \{v_1, v_2, \ldots, v_{|\mathcal{L}|}\}$ the set of   reference views selected up to the current step. This means that $v_{|\mathcal{L}|}= v_{i-1}$ at the $i$-th step. Also, since we impose $v_i>v_{i-1}$ at each optimization step, we have   $v_1 < v_2 < \ldots < v_{|\mathcal{L}|}$. 

 {At the $i$-th optimization step, we can consider two   cases: i) all  viewpoints $u\inÊ[U_L, v_{i-1}]$   have the best right  reference view in $\mathcal{L}$; ii) at least one viewpoint  $[U_L, v_{i-1}]$  it is still looking for the best right view.  The latter case is experienced if 
\begin{equation}\label{eq:cond_UL}
\exists u\in [U_L, v_{i-1}] \text{ s.t. }\min_{\substack{V_L\leq u \leq V_R, \\ (V_L, V_R)\in \mathcal{L} }}d_u^s(V_L, V_R, D(V_L), D(V_R)) > \min_{\substack{V_L\leq u \leq V_R^{\prime}, \\  V_L \in \mathcal{L}, V_R^{\prime} >  v_{|\mathcal{L}|}}}
d_u^s(V_L, V_R^{\prime}, D(V_L), D(V_R^{\prime})) 
\end{equation}}
Note that, in both cases,   the left reference is selected within the views in  $\mathcal{L}$, since any other view $v_i$ will be greater than $u$.    Let $\Phi\left(U_L,  \mathcal{L}, k \right)$ be the best distortion experienced over the range $[U_L, U_R^0]$ given that views in $\mathcal{L}$ have been already selected as reference views and $k$ reference views still have to be selected in the range $[v_{|\mathcal{L}|}+\delta, \infty]$, where we recall that $v_{|\mathcal{L}|}$ is the most right view in $\mathcal{L}$.  While $U_L$ might vary at each iteration step, $U_R^0$ stays constant. Thus, we omit the dependency of  $\Phi$ on $U_R^0$.


%
% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=0.8\linewidth ,draft=false]{figure/iterative_step.eps} 
% \caption{Solving method at the $i$-th optimization step. }\label{fig:iterative_step}
% \end{center}
% \end{figure}
 
We are then interested in finding the best $v_i$ using the following recursion
\begin{align}\label{eq:optimal_1}
\Phi(U_L,\mathcal{L},k) &= \min_{v_i > v_{|\mathcal{L}|}} \left\{  \min\left[
\Phi(U_L, \{\mathcal{L} \cup v_i\}, k-1),  \right. \right. \\ \nonumber
&  \left. \left. 
\sum_{u=U_L}^{\tilde{v_i}} \min_{
\substack{   V_L\leq u\leq V_R: \\ V_L, V_R \in  \{\mathcal{L} \cup v_i\}}
}\{d_u^s(V_L,V_R,d(V_L),d(V_R))\} +  \Phi(v_i + \delta, \{\mathcal{L} \cup v_i\}, k-1)
\right] \right\}
\end{align}
where $\tilde{v_i}$ is the left-most view between $v_i$ and $U_R^0$, and
\begin{align}
\Phi(U_L,\mathcal{L}, 1)  & =  \min_{v_i \geq  v_{|\mathcal{L}|}}\left\{ \sum_{u=U_L}^{  U_R^0 } \min_{\substack{V_L\leq u\leq V_R: \\  V_L, V_R \in  \{\mathcal{L} \cup v_i\}}}
\{d_u^s(V_L,V_R,d(V_L),d(V_R))\}    \right\}    \nonumber
 \end{align}
and 
$$
\Phi(U_L^0,\emptyset, C)  =   {D}(\mathcal{T}^{\star},U_L^0, U_R^0)
$$
In the recursion in Eq. \eqref{eq:optimal_1} the two cases mentioned above are highlighted: if in the range $[U_L, v_i]$ there is at least one viewpoint that does not have the best right reference view in $\mathcal{L}\cup v_i$, then $\Phi(U_L,\mathcal{L},k)= \Phi(U_L,\mathcal{L}\cup v_i,k-1)$. However,  if all viewpoints in the range $[U_L, v_i]$ are best reconstructed with the views in $\mathcal{L}\cup v_i$, then the best distortion $\Phi(U_L,\mathcal{L},k)$  can be decomposed into the sum of the distortion at which each viewpoint in  $[U_L, v_i]$ is reconstructed, plus  $ \Phi(v_i + \delta, \{\mathcal{L} \cup v_i\}, k-1)$, which is the best distortion of the remaining range. 

To better understand the above recursion, we consider the example in Fig. \ref{fig:Distorted_B}, where region $[U_L^0,v_2]$ is reconstructed from views $(v_1,v_5)$, region $[v_2+\delta,v_3]$ from $(v_2,v_4)$, and $[v_3+\delta,v_4]$ from $(v_3,v_5)$.  This means that in the iteration we have $\Phi(U_L,\mathcal{L},k)  = \min_{v_i > v_{|\mathcal{L}|}}  \Phi(U_L, \{\mathcal{L} \cup v_i\}, k-1) $, for  the first four iterations. Then, at the fifth step, we will have $v_i=v_5$, $\mathcal{L}=\{v_1, v_2, v_3, v_4\}$,  and the range $[U_L^0, v_5]$ is such that all viewpoints can be reconstructed from left and right views in $\{\mathcal{L} \cup v_5\}$. Thus, $\Phi(U_L,\mathcal{L},k)=  \sum_{u=U_L}^{\tilde{v_i}} \min_{\substack{ V_L, V_R \in  \{\mathcal{L} \cup v_i\}: \\  V_L\leq u\leq V_R}}\{d_u^s(V_L,V_R,d(V_L),d(V_R))\} +  \Phi(v_i + \delta, \{\mathcal{L} \cup v_i\}, k-1)$.

The proposed algorithm is optimal, as proved in the following subsection.  To evaluate $\Phi(U_L^0,\emptyset, C)$, we need to construct a tree whose depth is equal to $C$ and each node at depth $i$ represents the reference view selected at the $i$-th step of the iteration. Since we have no a priori assumption on the distortion function and on the distortion of the reference views, we can decide the best view subsets only once the entire tree is constructed.   The complexity of the algorithm is then exponential, namely $\mathcal{O}(|\mathcal{U}|^C)$, where $C$ is the depth of the tree and  $|\mathcal{U}|$ is the maximum number of recursive calls per node.  



\note{In Appendix \ref{sec:appendix_D}, I formulate an alternative solving method still optimal and still  with exponential complexity. Basically it is the solving method that makes use of the segments. }
 

\subsection{Proof of Optimality}
\label{sec:sub:proof_optimality}
We now prove the optimality of the algorithm proposed in Eq. \eqref{eq:optimal_1}. 
The goal is to show that $\Phi\left(U_L^0, \emptyset,  C \right)$ is the best distortion experienced over the range $[U_L^0, U_R^0]$ given that  $C$ reference views are optimized.  We prove it by induction. 

We start by showing the optimality for $k=1$ for $\Phi\left(U_L, \mathcal{L},  1 \right)$. The optimality is straightforward  given that
\begin{align}\label{eq:opt_k1}
\Phi(U_L,\mathcal{L}, 1)  & =  \min_{v_i \geq  v_{|\mathcal{L}|}}\left\{ \sum_{u=U_L}^{  U_R^0 } \min_{\substack{V_L\leq u\leq V_R: \\  V_L, V_R \in  \{\mathcal{L} \cup v_i\}}}
\{d_u^s(V_L,V_R,d(V_L),d(V_R))\}    \right\}    \nonumber
 \end{align}
This means that $v_i$ is the most right reference view of the subset of reference views. We know that $\{\mathcal{L} \cup v_i\}$ is the best right reference views set for all viewpoints in the range $[U_L,U_R^0]$ since by definition at least one viewpoint beyond $U_L$ does not have a best right view in $\mathcal{L}$. Thus, the best right view it is not included in $\mathcal{L}$ and $v_i$ is defined such that $\{\mathcal{L} \cup v_i\}$ minimizes the distortion over the range $[U_L,U_R^0]$, which leads  exactly the minimization in Eq. \eqref{eq:opt_k1}. 

\vspace{2mm}
We now consider the case of $k>1$.  We assume that $\Phi\left(U_L, \mathcal{L},  k-1 \right)$ is optimal, i.e., it is the best distortion that can be experienced over the range  $[U_L, U_R^0]$ when $\mathcal{L}$ views have been already selected and $k-1$ reference views still have to be optimized in the   range beyond $v_{|\mathcal{L}|}$.  We then have two possibile cases: 
\
\newline
 \emph{Case 1):  not all viewpoints in   the current range have a right reference view in $\{\mathcal{L} \cup v_i\}$.} This means that we have 
\begin{align}
\Phi(U_L,\mathcal{L},k) &= \min_{v_i > v_{|\mathcal{L}|}} \left\{ 
\Phi(U_L, \{\mathcal{L} \cup v_i\}, k-1) \right\}
\end{align}
where $\Phi(U_L, \{\mathcal{L} \cup v_i\}, k-1)$ is the best distortion of the range $U_L,U_R^0$, given that $k-1$ reference views have to be selected larger than $v_i$ and that at least one viewpoint in  $[U_L, v_i]$ will be synthesized with   right reference larger than $v_i$. We then consider $v_i$ as the best view that minimizes $\Phi(U_L, \{\mathcal{L} \cup v_i\}, k-1)$. This means that    $\Phi(U_L,\mathcal{L},k)$ is the best distortion over $[U_L,U_R^0]$ given that $k$ views need to be selected beyond $v_{|\mathcal{L}|}$ and     the range $[U_L, v_i]$ is not entirely reconstructed from $\{\mathcal{L} \cup v_i\}$.
\
\newline
 \emph{Case 2):   all viewpoints in   the current range have a right reference view in $\{\mathcal{L} \cup v_i\}$.} This 
 means that we have 
\begin{align} 
\Phi(U_L,\mathcal{L},k) &= \min_{v_i > v_{|\mathcal{L}|}} \left\{     \sum_{u=U_L}^{\tilde{v_i}} \min_{
\substack{   V_L\leq u\leq V_R: \\ V_L, V_R \in  \{\mathcal{L} \cup v_i\}}
}\{d_u^s(V_L,V_R,d(V_L),d(V_R))\} +  \Phi(v_i + \delta, \{\mathcal{L} \cup v_i\}, k-1)
  \right\}
\end{align}
This means that we select $v_i$ such that the range $[U_L, U_R^0]$ has a minimum distortion, given   $k-1$ remaining views. This is true since $v_i$ divides the  range $[U_L, U_R^0]$ is two sub-ranges, namely $[U_L, v_i]$ and $[v_i+\delta, U_R^0]$. The distortion over  $[U_L, U_R^0]$ is then the sum of the distortion over the two ranges, where $[v_i+\delta, U_R^0]$ is reconstructed at the lowest distortion (because of the optimality of $\Phi(v_i + \delta, \{\mathcal{L} \cup v_i\}, k-1)$). For the range  $[U_L, U_R^0]$, we evaluate the distortion assuming that the range has  $\{\mathcal{L} \cup v_i\}$ as reference views set. We know that there at least one viewpoint in $[U_L, v_i]$ that has  $v_i$ as best right  view (for the definition of $U_L$ as the starting of the viewpoints looking for right view) and we know that there is no view larger than  $v_i$ that could be used, otherwise we would be in the Case 1) introduced above. This means that  that $\Phi(U_L,\mathcal{L},k)$ is the best distortion over $[U_L,U_R^0]$ given that $k$ views need to be selected beyond $v_{|\mathcal{L}|}$ and  $\{\mathcal{L} \cup v_i\}$  is   the right reference set for   the range $[U_L, v_i]$.
 
Among the two possible cases above, we will select the one that minimizes the distortion. This ensures that $\Phi(U_L^0,\emptyset, C)$ is the best distortion over $[U_L^0,U_R^0]$ given that $C$ views need to be selected between  $[0, \infty]$, which leads to $D(\mathcal{T}, U_L^0,U_R^0)$. 





==> discussion.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.65\linewidth ,draft=false]{figure/Lemma2.eps} 
\caption{Scenario considered in Lemma 2.}
\label{fig:Lemma2}  
\end{center}
\end{figure}

From the equivalence model derived above, we can then carry out rules on when it is worth  synthesizing in the network.

\vspace{3mm}

{\bf\emph{Lemma 1:}} If $\exists v_i\in \mathcal{U}   \setminus  \mathcal{V}, v_i \leq U_l$ such that $\hat{v}_i^l<v<U_L,   v\in  \mathcal{V}$, then synthesizing viewpoint $v_i $
 does not improve the performance. 
 Analogous for the   reference views $v_i \geq U_R$. \vspace{1.5mm}
\newline
Lemma 1 interests the lateral reference views and   states that any camera view $v$ closer to $U_L$ than $\hat{v}_i^l$ is preferred as reference view over $v_i$. Same can be stated if $v$ is distorted but $\hat{v}_i^l<\hat{v}^l$. This Lemma immediately derives from  the ``monotonicity in   reference view distance" and the ``distorted reference view equivalence". 

\vspace{3mm}

{\bf\emph{Lemma 2:}} 
Let $\{v_1, \ldots, v_i\}$ be the set of $i$ selected reference views. We are interest in selecting another reference view  between $[v_i,U_R]$.   Let $v_n \in\mathcal{U}\setminus\mathcal{V}$ and   $v_k \in \mathcal{V}$  be respectively synthesized and undistorted views that can be selected as additional reference view, with  $v_i< v_n <v_k <U_R$. If $\hat{v}_n^l < v_i$ and $\hat{v}_n^r > v_k$, there is no gain in synthesizing $v_n$ and   $v_k$ is preferred over the  $v_n$.  
 \vspace{1.5mm}
   
{\bf\emph{Lemma 3:}} 
Let $\{v_1, \ldots, v_i\}$ be the set of $i$ selected reference views. We are interest in selecting another reference view  between $[v_i,U_R]$. Let $v_n \in\mathcal{U}\setminus\mathcal{V}$ and   $v_k \in \mathcal{V}$  be respectively synthesized and undistorted views that can be selected as additional reference view, with  $v_i< v_k <v_n <U_R$. If $v_i <\hat{v}_n^l < v_k$, there is no gain in synthesizing $v_n$ since   $v_k$ is preferred over the  $v_n$.  
 \vspace{1.5mm}

Note that both Lemma 2 and Lemma 3 consider two specific cases ($v_k >v_n$ and $v_k <v_n$) and shows conditions under which the synthesized view is not preferred over the undistorted camera view. %As expected, the conditions depend on the position of the equivalent reference view. This means that the Lemmas shows when the synthesized viewpoint is too much distorted to be used as reference view for further synthesis.  
Proof of the Lemmas are given in   Appendix \ref{sec:appendix_A}. 

From the above Lemmas, we can identify cases in which synthesizing does not lead to any gain and sending original camera views is preferred. This knowledge helps the optimization steps, since it reduces the search space of the solution,  but it can also be used to design efficient systems. 
 


==> intro.tex <==
Interactive free viewpoint video systems \cite{tanimoto11} endow users with the ability to choose and display any virtual view of a 3D scene, given original viewpoint images captured by an array of closely spaced cameras. Each virtual view image can be synthesized by the decoder via \textit{depth-image-based rendering} (DIBR)~\cite{Fehn_C_2004} using texture and depth images of two neighboring viewpoints as reference. In a bandwidth-constrained network streaming scenario---called \textit{interactive multiview video streaming} (IMVS) in the literature \cite{Gene:J11}---one key challenge is to select an appropriate subset of reference views from a potentially large number of camera-captured views for transmission to a client, so that he / she can enjoy high quality, low interactive delay view navigation even in resource-constrained environments~\cite{LiuQinMaZha:J10,  Chack:J13,Toni:J14}. 
%is to correctly provide the requested viewpoint to final users, without an a priori model of users' demand. Ideally, all camera views should be sent to users, to allow a complete navigation of the scene.  This however  comes at a large price in terms of bandwidth that  cannot   usually be sustained by the network resources. To reduce the network usage, %camera views could be sent a posteriori (after receiving users' request).  The system however would suffer  of   large \ac{RTT}, which is the delay that incurs between the time in which a user  requests a new view and the time in which it is able to actually display the requested view, i.e., the time it receives optimal camera views to optimally perform DIBR are received.   
%
%To overcome these limitations, 
% only a subset of camera views can be sent to clients. However,%   when only a limited number of camera views can  be sent to clients, 
 % how to properly quantize the camera view space is still an open challenge  in  \acp{IMVS}. 
  %
%Although research has been carried out recently to  find the best delivery strategy to efficiently serve interactive users~\cite{Toni:C13,Gurler:J13,Gene:J11},    the rendering of virtual view is always considered    at the client side.  


In this paper, we propose a new paradigm to further improve the reference view selection performance.   %we propose a new paradigm where virtual viewpoints can be synthesized in the \blue{ cloud network} as new reference for transmission to the client. More precisely, 
We argue that, in the case where the available bandwidth is too small for transmitting all camera views necessary to synthesize virtual views in conventional systems, a better strategy consists in  \textit{re-sampling the viewpoints of the 3D scene}---synthesizing novel virtual views in the cloud  network, which are transmitted as new references to the decoder. In particular, we consider a hierarchical cloud framework, where intermediate proxies called \textit{cloudlets} between the central cloud and the end users \cite{Verbelen:2012,Satyanarayanan:J09} perform customized reference view selection per user. % See Fig. \ref{fig:ConsideredScenario} for an illustration. 
In general, service personalization at cloudlets %proxies\footnote{Proxy-based service also means computation load at the centralized server is greatly relieved.} 
instead of the main cloud means a smaller \ac{RTT}, hence more reactive systems.  \note{Do we still want to consider an example in which we better justify the proxy server and last-hop mile bottleneck?}
%In the following,  we consider the case where cloudlets instances are represented as proxy server.   


\begin{figure}[t]
\begin{center}
\includegraphics[width=1\linewidth,draft=false]{figure/ConsideredScenario_V5.eps}
\caption{Considered scenario. Green lines represent no bandwidth constrained channels, red lines are bottleneck channels.}
\label{fig:ConsideredScenario}
\end{center}
\end{figure}

In more details, we consider a distributed architecture where the interactive free viewpoint service is provided by a network of cloudlets at the edges of the core network, as shown in Fig.~\ref{fig:ConsideredScenario}. A main cloud   stores  pre-encoded  free viewpoint video in camera viewpoints. The coded cameras are transmitted to the edge cloudlets that act as proxies for final delivery to clients. Each cloudlet sends to a client the set of reference view that enable synthesis of all viewpoints in the client's navigation window. The latter is considered as the range of viewpoints in which the user can navigate during the RTT. This ensures zero-delay during view-switching. We assume there is sufficient network capacity between the main cloud and the edge cloudlets for the transmission of \blue{all   camera views}. There exists however a bottleneck of limited capacity  between %a client and the corresponding  proxy
\blue{a cloudlet and a nearby user}  \footnote{In practice, the last-mile access network is often the bottleneck in real-time media distribution.}. Because of the bottleneck,   the \blue{cloudlet} is unable to continuously transmit all camera views in the navigation window.  Hence, each \blue{cloudlet} must select or construct  a small set of reference views  for transmission to the user depending on its interaction with the system such that the quality of the navigation is optimized.   %The possible viewpoints offered to the users are denoted as   $\mathcal{U} = \{u_1, u_{1+\delta}, \ldots, u_N\}$.  It contains synthetic views and camera views  for navigation   between leftmost and rightmost camera views $v_1$ and $v_N$. It is equivalent to offering views $u=k\delta$,  where $k$ is a positive integer and $\delta$ is a pre-determined fraction that describes the minimum view spacing between neighboring virtual views. In particular, we assume that a virtual view can have a non-integer index $i.x$, which corresponds to a position between camera views $v_i$ and $v_{i+1}$.   We consider   that any virtual viewpoint  $u\in\mathcal{U}$ can be synthesized using a pair of left and right reference view images $v_L$ and $v_R$, $v_L < u < v_R$, via a known DIBR technique such as 3D warping\footnote{Note views synthesis can be performed at the source side (to generate reference views) but also at the client side (to reconstruct the range of interest). In both cases, the same rendering method and distortion model apply. }~\cite{Mori200965}.    The proxy needs to optimize  the best subset of $C$  viewpoints in  $\mathcal{U}$ that maximize the navigation quality of the client. 
   We argue that in  resource-constrained networks, a view re-sampling strategy in the \blue{cloudlet, and so in the network} is beneficial compared to the mere subsampling of the original set of camera views.   We illustrate this in   Fig.~\ref{fig:ConsideredScenario}, where the main \blue{cloud}  stores three coded camera views: $\{v_1, v_2, v_3\}$ while  the bottleneck links between \blue{cloudlet}-user pairs can support the transmission of only two views.    In particular, we consider integer index $i$ for any the camera view,  while  we assume that a virtual view can have a non-integer index $i.x$, which corresponds to a position between camera views $v_i$ and $v_{i+1}$.    If \blue{user} 1 requests navigation window $[u_{2.4}, u_{2.8}]$, the   \blue{cloudlet} can simply forward the closest camera views $v_2$ and $v_3$. However, if \blue{user} 2 requests the navigation window $[u_{1.8}, u_{2.2}]$, transmitting camera views $v_1$ and $v_3$ results in large synthesized view distortions due to the large distance between reference and virtual views (called \textit{reference view distance} in the sequel). Instead, the \blue{cloudlet} can synthesize virtual views $u_{1.8}$ and $u_{2.2}$ using camera views $v_1, v_2, v_3$ and send them to the \blue{user} 2 as new reference views for the virtual view window $[u_{1.8}, u_{2.2}]$. Because of the smaller reference view distance, this strategy may result in smaller synthesized view distortion. However, the virtual view synthesis process introduces distortion into the new reference views $u_{1.8}$ and $u_{2.2}$. This tradeoff has to be carefully considered when choosing which views to synthesize at the proxy. \red{paragraph too long.}
 
Equipped with the above intuitions, we study   the main tradeoff   between reference distortion and bandwidth gain and we formulate a new   \emph{synthesized reference view selection optimization problem}.  It consists in  selecting the optimal  reference views  that lead to the minimum distortion for all synthesized virtual views in \blue{the user's navigation window} to a bandwidth constraint between the proxy and the client.   The main novelty in the optimization framework lies in the possibility for the edge server  to transmit  synthesized viewpoints as reference views and not only original camera views.  We show that this combinatorial problem can be optimally solved but that it is NP-hard. We then introduce an assumption on the view distortion that is   in most of the 3D video sequences. With this assumption, the optimization problem can be solved in polynomial time by a \ac{DP} algorithm.  This endows us with an efficient algorithm to study the reference view selection problem when synthesis is allowed in the network.  We then provide simulation results,    carried out   for synthetic \red{I think u mean synthetic here, i.e., not real} \note{yes, do we leave synthetic?} and natural sequences. They demonstrate  the quality gain experienced by the IMVS system  when synthesis is allowed in the network with respect to scenarios whose edge servers can only transmit camera views. \blue{ They also show that synthesis in the network allows to maintain good navigagtion quality when reducing the number of acquiring cameras as well as when non-optimally placed cameras are considered. 
% adopting synthesis in the network can compensate for non properly located camera views in the 3D scene, which
This  is an important advantage in practical settings.}% \red{I don't get the last point.} 


 
The remainder of this paper is organized as follows. Related works   are described in Section \ref{sec:related}.   The reference view selection optimization problem is then formulated in Section \ref{sec:algo}.  In Section \ref{sec:sys_overview}, we provide a   system overview and basic intuitions on the gain in synthesizing in the network.  The polynomial time view selection  algorithm  is described in Section \ref{sec:algo_approx}.   In Section \ref{sec:results}, we discuss the simulation results, and we conclude in Section \ref{sec:conclusion}.

 
 
 
 
 
 
 

==> intro_old.tex <==
In free viewpoint video systems, given a set of images captured by a set of closely spaced cameras, an intermediate virtual view image can be synthesized by the decoder via \textit{depth-image-based rendering} (DIBR)~\cite{Fehn_C_2004}, using two camera-captured viewpoint images to the left and right respectively as reference. This   has led to an increasing interest in new \ac{IMVS}, where  users have the ability to choose and display any virtual viewpoint of a 3D scene,  originally acquired by  an array of cameras. One of the main challenge in \ac{IMVS} is to correctly provide the requested viewpoint to final users, without an a priori model of users' demand. Ideally, all camera views should be sent to users, to allow a complete navigation of the scene.  This however  comes at a large price in terms of bandwidth that  cannot   usually be sustained by the network resources. To reduce the network usage, %camera views could be sent a posteriori (after receiving users' request).  The system however would suffer  of   large \ac{RTT}, which is the delay that incurs between the time in which a user  requests a new view and the time in which it is able to actually display the requested view, i.e., the time it receives optimal camera views to optimally perform DIBR are received.   
%
%To overcome these limitations, 
 only a subset of camera views can be sent to clients. However,%   when only a limited number of camera views can  be sent to clients, 
  how to properly quantize the camera view space is still an open challenge  in  \acp{IMVS}. 
  
Although research has been carried out recently to  find the best delivery strategy to efficiently serve interactive users~\cite{Toni:C13,Gurler:J13,Gene:J11},    the rendering of virtual view is always considered    at the client side.  In this paper,   we argue  that, in the case where the available bandwidth is too small for the server to transmit all camera views conventionally used to synthesize virtual views in the navigation window, there exists a better strategy than simply transmitting a subset from $N$ available camera views as reference for client-side view synthesis. Instead, \textit{one can re-sample the viewpoints of the 3D scene} and synthesize intermediate virtual views as new references to be transmitted to the decoder, so that the synthesized view distortion within the navigation window is further minimized. In particular, we consider a distributed proxy architecture, where an interactive free viewpoint service is provided by a network of \textit{proxies} at the edges of the core network, as shown in Fig.~\ref{fig:ConsideredScenario}. A distant server has pre-encoded and currently stored a free viewpoint video in $N$ camera viewpoints $\mathcal{V} = \{1, \ldots, N\}$. The feasible range $\mathcal{U} = \{1, 1+\delta, \ldots, N\}$ of synthesized virtual views $u = k \, \delta$ for navigation is between leftmost and rightmost camera views $1$ and $N$, where $k$ is a positive integer and $\delta$ is a pre-determined fraction that describes the minimum view spacing between neighboring virtual views. 

 \begin{figure}[t]
\begin{center}
\includegraphics[width=0.8\linewidth,draft=false]{figure/ConsideredScenario_V3.eps}
\caption{Considered scenario. Dashed lines represent no bandwidth constrained channels, solid lines are bottleneck channels.}
\label{fig:ConsideredScenario}
\end{center}
\end{figure}
 
When a client initiates an interactive streaming session, the requested $N$-view video is first pre-fetched (if not locally cached) to a proxy that directly serves the clients. In general, service personalization at proxies\footnote{Proxy-based service also means computation load at the centralized server is greatly relieved.} instead of server means a smaller \ac{RTT} and hence a smaller navigation window $W$. With a \ac{RTT} of $T$ seconds between the proxy and the client, and a maximum speed $\rho$ at which a user can navigate to neighboring virtual views, one can compute a \textit{navigation window} $W(u) = [u-\rho T,u+\rho T]$, given that the user has selected virtual view $u$ at some time $t_0$. By transmitting reference views for synthesis of virtual views in $W(u)$ at time $t_0 + T/2$, the client can experience zero-delay view navigation at time $t_0 + T$ (see \cite{xiu12} for details). However, there often exists a bottleneck link between proxy and client\footnote{In practice, the last-mile access network is often the bottleneck in real-time media distribution.}, such that the proxy is unable to continuously transmit $N$ camera views to the client. Hence, each proxy must select or construct $M < N$ reference views for transmission to the client depending on its interaction with the system.



In this bottleneck network, a re-sample strategy can be beneficial, as shown in the following example. The server in Fig.~\ref{fig:ConsideredScenario} stores three coded camera views: $\{1, 2, 3\}$ and  the bottleneck links between proxy-client pairs can support transmission of only two views. We assume that a virtual view can have a non-integer index $i.x$, which corresponds to a position between camera views $i$ and $i+1$. If client 1 requests navigation window $[2.4, 2.8]$, the servicing proxy can simply forward the closest camera views $2$ and $3$. However, if client 2 requests navigation window $[1.8, 2.2]$, transmitting camera views $1$ and $3$ results in large synthesized view distortions due to the large distance between reference and virtual views (called \textit{reference view distance} in the sequel). Instead, the proxy can synthesize virtual views $1.8$ and $2.2$ using camera views $1,2,3$ and send them to the client 2 as new reference views for the virtual view window $[1.8, 2.2]$. Because of the smaller reference view distance, this novel strategy may result in smaller synthesized view distortion. However, the virtual view synthesis process introduces distortion into the new reference views $1.8$ and $2.2$. This tradeoff has to be carefully considered when choosing which views to synthesize at the proxy.



%For example,  in the scenario depicted in Fig. \ref{fig:ConsideredScenario},   a source node (either the   main  or the edge servers) has a set of  camera views $\mathcal{V}$  stored in its own cache.   While the main server communicates to edge server through a no-constrained channel,  each edge server  communicates to a receiver  through a dedicated channel with a constrained capacity.    Each user's request  is predicted at the source and identified by a viewpoint range.  Any viewpoint in this range can be synthesized if a left and right reference view is available at the receiver side.   
%Assuming that  the camera views at the edge server are $\mathcal{V}=\{1,2,3\}$, where views are indexed accordingly to their position, and that the channel allow at most a transmission of two reference views per time unit,  the IMVS cannot efficiently satisfy the request of user $1$, interest in displaying the range of viewpoints $[1.8,2.2]$. While viewpoints in $[1.8,2]$ is reconstructed best from camera views $(1,2)$, the ones in $[2,2.2]$ can be efficiently synthesized from the pair $(2,3)$. Thus, when quantizing the camera views and selecting only two of them, the client will not be properly satisfied. At the same time, the transmission of all three camera views would take  two transmission units, leading too large RTT for online IMVS applications. 


 
%How to efficiently reach this goal is still an open question since users' requests are not known a priori and  they are  usually  predicted  at the source. To compensate for this uncertainty,   a large number of camera views should be delivered to clients, coming at a large price in terms of bandwidth.  This challenge has been   investigated in few recent works, aimed at finding the best delivery strategy to efficiently serve interactive users~\cite{Toni:C13,Gurler:J13,Gene:J11}, assuming that the rendering of virtual view is efficiently implemented at the client side. However, synthesizing at the client requires to send two reference frames per viewpoint. These might not be always feasible in networks with limited resources.% To   offload  clients' terminals (in terms of complexity), view synthesis in the network has been introduced  for cloud networks \cite{Wen:J13,Melodia:J13}. The desired view is synthesized in the cloud and then sent directly to clients.   However, only the  view requested by the client is synthesized. This means that either the desired view is a priori known  at the source or a switching delay is experienced by the clients.  


 
%
%We study the system provided in  Fig. \ref{fig:ConsideredScenario} and we focus on the optimization that each edge server has to perform to evaluate the best subset of  views to send to clients. Rather than limiting this reference views selection to camera views, we assume that also synthetic viewpoints can be selected. We show that for bottleneck channels, synthesizing at the server rather than at the client can partially overcome network constraints limitations. In the example of  Fig.  \ref{fig:ConsideredScenario},  %for example, we assume that both nodes A and B have received camera views $\mathcal{V}=\{1,2,3\}$, where views are indexed accordingly to their position. % Client $1$ and client $2$ are interested in the viewpoint ranges $[2.4, 2.8]$ and $[1.8, 2.2]$, respectively. We also assume that the channel links from nodes A  and B  to clients $1$ and $2$ allow  to send two views only.  While the first client can cover entirely his range of interest receiving camera views $\{2,3\}$, the second client would ideally need $\{1,2,3\}$ to navigate in the range of interest at the highest quality. However, because of bandwidth constraints, only   $\{1,3\}$ would be sent to entirely cover any viewpoint in the requested range. 
%if we  perform synthesis at the source  sending virtual viewpoints to clients, the edge server  B would  send to client $2$ viewpoints   $\{1.8, 2.2\}$, rather than camera views $\{1, 3\}$. Note that although viewpoints are distorted (because synthesized), they encapsulate the information of three camera views in two single viewpoints. This leads to a bandwidth gain at the price of a distortion in the reference views that are sent. 
%If $\{1.8, 2.2\}$ are virtually reconstructed  at high quality, client $2$  reconstructs the range $[1.8,2.2]$  at a better distortion using $\{1.8, 2.2\}$ as reference views rather than  $\{1,3\}$.  
 



We  investigate  the main tradeoff in IMVSs between reference distortion and bandwidth gain, by  
proposing a \emph{synthetic reference view selection optimization problem}.  We study the problem of selecting the optimal $M$ reference views---ones that lead to the minimum distortion for all synthesized virtual views in window $W(u)$ subject to a bandwidth constraint---for the proxy to transmit.   The main novelty in the optimization lies in the possibility for the edge server to send not only camera views but also synthesized viewpoints as reference views.   To study this reference view selection problem,  we  formulate a combinatorial optimization problem to find this best set of $M$ reference views under the assumption that the distortion of synthesized viewpoints respect a clearly stated assumption. We show that this problem can be optimally solved but it is NP-hard. We then introduce a second assumption for the distortion model,   valid in most of the 3D video sequences. Under these two assumptions, the optimization problem can be solved by a \ac{DP} solving method in polynomial time.  This endows us with an efficient algorithm to study the reference view selection problem when synthesis is allowed in the network.  We then provide simulation results,    carried out both from experimental and synthetic sequences. First, we experimentally prove the quality gain experienced by the IMVS when synthesis is allowed in the network, respect to scenarios in which edge servers can only transmit camera views. Then, we prove the benefit for a system designer in adopting synthesis in the network, showing for example that synthesis in the network can compensate for non properly located camera views in the 3D scene. 


The remainder of this paper is organized as follows. Related works on IMVS are described in Section \ref{sec:related}. Section \ref{sec:model} describes the  system model as well as the distortion model that describes the resulting distortions for synthetic viewpoints. The reference view selection optimization problem is then formulated at the end of the section. In Section \ref{eq:np_hard_proof} we provide the  NP-Hard proof. The simplified algorithm, solvable in polynomial time is described in Section \ref{sec:algo_approx}.   In Section \ref{sec:results}, we discuss the simulation results, and we conclude in Section \ref{sec:conclusion}.

 
 
 
 
 
 
 

==> model_old.tex <==
%\blue{We now describe the synthetic view selection problem introduced previously.  First, we provide a system model to specify our considered application scenario. Then, we present an image distortion model that models the resulting distortions of virtual view images synthesized using (possibly distorted) known left and right reference views. Finally, we formulate mathematically a succinct combinatorial optimization problem.
%}

\subsection{System Model}

As discussed in the Introduction, we consider the scenario depicted in Fig.\;\ref{fig:ConsideredScenario}, where a central source (main server) has pre-stored a piece of free viewpoint video content, captured from a set of $V$ camera views $\mathcal{V}=\{1,2, \ldots, V\}$. Specifically, we assume that there exist texture and depth maps at each camera-captured view, and each texture / depth map pair is encoded at the same rate using standard video coding tools like H.264\cite{wiegand03} or HEVC\cite{sullivan12}. These camera views are first sent to a network of intermediate edge servers. We assume that there is sufficient network capacity between source and edge servers for the transmission of all $V$ texture / depth map pairs, but from each edge server to a client $i$ there exists a bottleneck of limited capacity $C_i$, expressed in number of views.
We assume also that each edge server is capable of synthesizing viewpoints via DIBR; we denote by  $\mathcal{U}=\{1, 1/L, 2/L, \ldots, V\}$ the set of all viewpoints that can be potentially generated from $\mathcal{V}$ by the edge server. Note that $\mathcal{U}$  includes  both original camera views and synthesized virtual viewpoints, where the camera views are indexed by integer numbers and virtual views are indexed by non-integer values.    

We assume that interactive clients request viewpoints within the range $[1,V]$. Specifically, a user $i$ requests viewpoint $u_i(t_o)$ from the edge server, $1\leq u_i \leq V$, at time $t_o$. Assuming a non-negligible round-trip time (RTT) delay of $T$ seconds between the edge server and the client, by the time the edge server has received the request and transmits corresponding left and right reference views to synthesize virtual view $u_i(t_o)$, the client will receive the needed reference data at time $t_o + T$, or $T$ seconds after the request for view $v_i(t_o)$ is sent. Thus, to enable zero-delay view-switching at the client, the edge server, upon receiving request for virtual view $v_i(t_o)$ at time $t_o + T/2$, should transmit reference views to enable synthesis of any virtual view in \textit{navigation window} $[u_i(t_o) - \rho T, u_i(t_o) + \rho T]$, where $\rho$ is the maximum speed at which a client can navigate to neighboring virtual views.

More generally, we denote the navigation window of a client $i$ by $[U_{L,i}^{0}, U_{R,i}^{0}]$, within which the edge server needs to provide reference data for virtual view synthesis. If bandwidth is not a concern, ideally the edge server should send to client $i$ the union of all left and right reference views in $\mathcal{V}$ that synthesize the best quality virtual view $u_i$, $\forall u_i \in [U_{L,i}^{0}, U_{R,i}^{0}]$. When this is not feasible due to limited bandwidth $C_i$, the edge server needs to select the best subset $\mathcal{U}' \subset \mathcal{U}$ such that the aggregate distortion of all virtual views $u \in [U_{L,i}^{0}, U_{R,i}^{0}]$ is minimized and $|U'| \leq C_i$. If $\mathcal{U}'$ contains non-camera views, it means that the edge server needs to synthesize virtual viewpoints as new reference for client-side virtual view synthesis.

In the following, we formulate a reference view selection optimization that can be solved at each server for client $i$, given navigation window $[U_{L,i}^{0}, U_{R,i}^{0}]$.
  
  

\subsection{Assumptions on Synthesized View Distortion}
\label{sec:sub:View_Distortion}

We now discuss two assumptions on the synthesized view distortion function that we will exploit in the algorithm development section for fast computation. We assume first that any virtual viewpoint  $u\in\mathcal{U}$ can be synthesized using a pair of left and right reference view images $v_L$ and $v_R$, $v_L < u < v_R$, via a known DIBR technique such as 3D warping\footnote{Note views synthesis can be performed at the source side (to generate reference views) but also at the client side (to reconstruct the range of interest). In both cases, the same rendering method and distortion model apply. }~\cite{Mori200965}.  %The distortion of the synthesized image of virtual view $u$ depends on: i) the distances between $u$ and the reference views, \textit{i.e.} $|u - v_L|$ and $|v_R - u|$, and ii) the distortions of the reference views. 
We denote by  $d_u(v_L,v_R, D_L,D_R)$ the distortion of the virtual view $u$ synthesized from the left and right reference views $v_L$ and $v_R$ with respective distortions $D_L$ and $D_R$. The first assumption on synthesized view distortion $d_u(\,)$ is \textit{shared optimality of reference views}: 

\subsubsection{Shared optimality of references for virtual viewpoints}      

\begin{align}\label{eq:shared_optimality}
&\text{if } d_u(v_L,v_R, D(v_L),D(v_R)) \leq d_u(v_L^{\prime},v_R^{\prime}, D(v_L^{\prime}),D(v_R^{\prime}))  
  \\  \nonumber
&\text{then } d_{u'}(v_L,v_R, D(v_L),D(v_R)) \leq d_{u'}(v_L^{\prime},v_R^{\prime}, D(v_L^{\prime}),D(v_R^{\prime}))  
\end{align}
for $\min\{v_L,v_L^{\prime}\} \leq u, u' \leq \min\{v_R,v_R^{\prime}\}$. In words, (\ref{eq:shared_optimality}) states that if the virtual view $u$ is better synthesized from the reference pair $(v_L,v_R)$  than from $(v_L^{\prime},v_R^{\prime})$, then  $u^{\prime}$ is also better synthesized from $(v_L,v_R)$, given both reference pairs are candidate reference pairs for $u$ and $u^{\prime}$.  This assumption is justified in conventional 3D video sequences, as shown in Appendix \ref{sec:appendix_B}. %characterized by foreground objects over a background. In particular, when foreground objects are not too close to the acquiring cameras and the background is not highly heterogeneous, the distortion of synthetic viewpoints has in general an increasing behavior with both the distance of reference view from the viewpoint or the reference view distortion. As formally discussed in   Appendix \ref{sec:appendix_B}, for these conventional 3D images the assumption of shared optimality of references for virtual viewpoints is respected. 

The second assumption on synthesized view distortion $d_u(\,)$ is \textit{independence of reference optimality}.

\subsubsection{Independence of optimality for left and right references}      
\begin{align}\label{eq:indep_optimality}
&\text{if } d_u(v_L,v_R, D(v_L),D(v_R)) \leq d_u(v_L^{\prime},v_R, D(v_L^{\prime}),D(v_R))  
  \\  \nonumber
&\text{then } d_u(v_L,v_R^{\prime}, D(v_L),D(v_R^{\prime})) \leq d_u (v_L^{\prime},v_R^{\prime}, D(v_L^{\prime}),D(v_R^{\prime})). 
\end{align}
In words, (\ref{eq:indep_optimality}) states that if the virtual view $u$ is better synthesized from  $v_L$ is a better left reference than $v_L'$ for virtual view $u$ in combination with right reference $v_R$, then $v_L$ remains better as left reference for $u$ even if some other right reference $v_R'$ is use in combination. 
Also this second assumption is valid in more of the 3D video sequences, as shown in Appendix \ref{sec:appendix_B}. \note{I refer to the Appendix to justify these assumptions. Is it OK?} %In particular, for the condition not to hold the scenario has to be such that one right reference view is complementary (in terms of reconstructed region in the DIBR) to a given left reference view and not almost overlapping to any another left reference view.

 

\subsection{Problem Formulation}

We assume that each camera-captured view $v \in \mathcal{V}$ is distorted only by lossy compression with resulting distortion $d(v)$. Among the viewpoints in $\mathcal{U}$, the edge server selects a subset ${\mathcal{T}}_{i} \subseteq \mathcal{U}$ to send to client $i$ such that the distortion $\mathcal{D}({\mathcal{T}}_{i})$ experienced over the navigation window is minimized and network constraints are met. Distortion $\mathcal{D}(\mathcal{T}_{i})$ for client $i$ can be written as:
\begin{align}\label{eq:distortion_user}
\mathcal{D}({\mathcal{T}}_{i}) = \sum_{u\in[U_{L,i}^{0}, U_{R,i}^{0}]}  \min_{v_L, v_R \in {\mathcal{T}}_{i}} \left\{ d_u(v_L,v_R, D(v_L),D(v_R)) \right\} 
\end{align}
where $D(v_L)$ and $D(v_R)$ are the respective distortions of the left and right reference views. In (\ref{eq:distortion_user}), for each virtual view $u$ the best pair of references in ${\mathcal{T}}_{i}$ are selected for synthesis. Note that the best reference pair may not be the closest references since the quality of $u$ depends not only of the distance between viewpoints and reference view, but also on their distortion. 
%Note also that a lossless channel is considered. Furthermore, because of timing constraints, views that are not selected in ${\mathcal{T}}_{i}$ cannot be sent at successive transmission opportunities. 
 
We can now formalize our combinatorial optimization as follows. Given a navigation window $[U_{L}^{0}, U_{R}^{0}]$ of a target client, we seek the optimal subset $\mathcal{T}^{*} \subseteq \mathcal{U}$ that minimizes $\mathcal{D}(\mathcal{T}^*)$ subject to transmission constraint $|\mathcal{T}| \leq C$:
\begin{align}\label{eq:optimization}
{{\mathcal{T}}}^{\star} :  &\arg \min_{{\mathcal{T}}}  \mathcal{D}({\mathcal{T}}) \\
\nonumber
 &\text{s.t }  | {{\mathcal{T}}} |\leq C \\ 
\nonumber
& \hspace{5mm}{{\mathcal{T}}}\subseteq \mathcal{U} 
\end{align}
We note that (\ref{eq:optimization}) differs from previous reference view selection formulations~\cite{Maugey:C14,DeAbreu:C14,ren15} in that the edge server has the extra degree of freedom to synthesize novel view(s) as new reference(s) for transmission to the client. 


\subsection{Graphical Representation of Reference Selection}
\label{subsec:graphical}

% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=0.65\linewidth ,draft=false]{figure/Undistorted_Region.eps} 
% \caption{Covering region in the case of distorted views.}\label{fig:Undistorted_Region}
% \end{center}
% \end{figure}
%%
%If we assume ``monotonicity in the distance", then the distortion in Eq. \eqref{eq:distortion_user} becomes
%\begin{align}\label{eq:distortion_user_3}
%\mathcal{D}({\mathcal{T}},U_L^0, U_R^0) = \sum_{i=1}^{C-1} \sum_{u=\tilde{v}_i}^{\tilde{v}_{i+1}}    d^s_u(v_i,v_{i+1}) \,.
%\end{align}
%with $\tilde{v}_1=U_L^0$,   $\tilde{v}_{C}=U_R^0$,  and  $\tilde{v}_c=v_c$ otherwise.
% Thus, any viewpoint $u$ is virtually synthesized best from the closest reference views on the left and on the right. A graphical representation of the reference views selection per viewpoint is provided in Fig. \ref{fig:Undistorted_Region} for the case of $5$ selected reference views.   
%In this case, the problem optimization in Eq. \eqref{eq:optimization}
% can be solved by dynamic programming based on the following recursion
%\begin{align}\label{eq:SM_nodist}
%\Phi(U_L,V_L,k) =\min_{v_i\in \mathcal{V} \mid v_i \geq U_L }\left\{   \sum_{u\in[U_L,v_i]} d^s_u(V_L,v_i) + \Phi(v_i+\delta, v_i,k-1)  \right\}    \,.
%\end{align}
%
 

 
 \begin{figure}[t]
\subfigure[]{
 \includegraphics[width=0.45\linewidth ,draft=false]{figure/Distorted_Region_A.eps} 
 \label{fig:Distorted_A}
 }
 \hfil
\subfigure[]{
 \includegraphics[width=0.45\linewidth ,draft=false]{figure/Distorted_Region_B_3.eps} 
 \label{fig:Distorted_B}
 }
 \hfil
 \subfigure[]{
 \includegraphics[width=0.45\linewidth ,draft=false]{figure/Distorted_Region_C.eps} 
 \label{fig:Distorted_C}
 }
 \hfil
 \subfigure[]{
 \includegraphics[width=0.45\linewidth ,draft=false]{figure/Distorted_Region_D.eps} 
 \label{fig:Distorted_D}
 }
 \hfil \caption{Covering regions in the case of undistorted views. Case (a) contradicts the shared reference. Case (b) contradicts the independence of optimality for left and right reference view. Cases (c) and (d) are feasible solutions under both assumptions.}\label{fig:Distorted_Region}
 \end{figure}
%
 

 
Optimization in \eqref{eq:optimization} selects a pair of reference views for each virtual view in the navigation window. We can graphically illustrate the selected reference views for virtual views in the window as shown in Fig.\;\ref{fig:Distorted_Region}. In the figure, the $x$-axis represents the virtual views in the navigation window $[U_L^0, U_R^0]$ that require synthesis. Correspondingly, the $y$-axis represents the reference views selected for synthesis of each virtual view $u$ in the navigation window; \textit{i.e.}, for each $u \in [U_L^0, U_R^0]$, there must either be selected reference pair $(v_L, v_R)$ such that $v_L < u < v_R$, or there is a selected reference $v = u$, in which case $v$ can be used directly as virtual view $u$ with no view synthesis. A horizontal line segment---\textit{e.g.}, $v=v_1$ for $U^0_L \leq u \leq v_3$ in Fig.\;\ref{fig:Distorted_A}---means the same reference is used for a range of virtual views. As shown, this graphical representation results in two step functions above and below the $u=v$ line, representing the selected right and left reference views respectively. The set of selected reference views are the union of the distinct step locations of the two step functions. 

%A black solid line for $v_i$ for all viewpoints in the range $[u_L,u_R]$ means that view $v_i$ is selected as reference view for that range.   Fig. \ref{fig:Distorted_Region} depicts the feasible solution spaces for  distorted reference views. In particular, for each $u$, one left and right reference view is selected above and below the $u=v$ line respectively. This satisfies the condition $V_L\leq u \leq V_R$. However, no other constraints are imposed. For example, the closest reference view might not be the optimal one for virtually synthesizing a viewpoint. This usually happens if the closest reference view  is much more distorted than a more far a part reference view.  Among all cases depicted in  Fig. \ref{fig:Distorted_Region}, we are interested in understanding which are the feasible scenarios under the distortion assumptions discussed in Sec. \ref{sec:sub:View_Distortion}.


This graphical representation of selected references is very useful in visualizing different kinds of solutions to \eqref{eq:optimization}. For example, under the assumption of shared reference optimality as discussed in Section \ref{sec:sub:View_Distortion}, we see that the selected reference views in Fig.\;\ref{fig:Distorted_A} cannot be an optimal solution. Specifically, virtual views $v_3 - 1/L$ and $v_3 + 1/L$ employ references $[v_1, v_4]$ and $[v_2, v_5]$ respectively.  However, if references $[v_1, v_4]$ are better than $[v_2, v_5]$ for virtual view $v_3 - 1/L$, they should be better for virtual view $v_3 + 1/L$ also according to shared reference optimality in \eqref{eq:shared_optimality}.

If the assumption of independence of reference optimality is additionally considered, 
then the reference view selection in Fig.\;\ref{fig:Distorted_B} is also not an optimal solution. Specifically, we see that both $v_3$ and $v_4$ are feasible right reference view for virtual views $v_3 - 1/L$ and $v_3 + 1/L$. Regardless of which left references are selected for these two virtual views, if $v_3$ is a better right reference than $v_4$, then both virtual views would select $v_3$ or vice versa. In contrast, reference view selections in Fig.\;\ref{fig:Distorted_C} and Fig.\;\ref{fig:Distorted_D} are candidate optimal solutions to \eqref{eq:optimization}.
 
 




==> related_old.tex <==
%% Cloud-service providers will be able to monetise their infrastructure through leveraging the increased demand for strategically located in-network media processing. 


Past works on multimedia streaming and cloud-services have shown the benefit of strategically located in-network media processing nodes in face of limited network resources, large network/users diversity, and limited computational complexity at the clients, highlighting the benefits in  jointly optimizing both source  processing and media delivery strategies in multimedia services \cite{Akyl:J07,Bacc:J14}.  In the following, we   provide the most significant works on in-network processing media, %showing its advantage in multimedia communications and cloud computing services, 
highlighting  however the lack of in-network processing for multi-view systems. %Then, we describe  main works on multiview reference frames optimization and coding strategies, showing the main differences between the published works and our contribution.

In-network media processing methodologies can be  mainly categorized in i) processing at the packet-level with no processing of the source information and ii) processing at the source level. In  the former class,  packet filtering,  routing strategies   \cite{De_Vleeschouwer:J07, Huang:C12}  or  caching of media content information \cite{Borst:C10,JiCaire:arxiv13}  allow to save network resources still maximizing the quality experienced by clients. To better address media delivery services in highly heterogenous scenarios,   network coding strategies  for multimedia streaming have been also optimized\cite{Dimakis:J10,Magli:J13,Vukob:J14}. Finally, in novel cloud computing media services, processing in the network can be beneficial for delay-sensitive applications. In particular, offloading to a resource-rich machine in the proximity of the device rather than in the cloud might reduce the transmission latency \cite{Tel_Schaar:C14}.
  
For the second class of in-network processing, the main objective is usually to avoid transmitting large amounts of raw streams to the clients  by processing the source data in the network to reduce both the communication volume and the processing required at the client side.  Transcoding strategies might be collaborative performed in peer-to-peer networks \cite{Wu_Huang:J11}  or in the cloud \cite{wen:J14}. Furthermore, source data can be compressed in the cloud \cite{Wu_Huang:J11,Huang_Mei:C11,Yue:J13} to efficiently address users' requests. Also, source redundancy spreading within the network might be opportunistically compressed for a better usage of network resources without jeopardizing users' service \cite{Sardari:C13}.  


However, to the best of our knowledge, none of the work investigating in-network media processing have considered multi-view interactive streaming.  So far most of the works in multiview streaming have been focused on the efficient design of representation methods for multiview data \cite{salvador:J13,Maug:Arxiv14},  efficient  transmission strategies of multi-camera networks, \cite{Chack:J13,Toni:J14,Fuji:J14}  assuming view-rendering to be performed at the client side.  However, allowing view-rendering in the network or in the cloud might lead to a better usage of both network resources and client limited capability in computation.  In this direction, to  offload  clients' terminals (in terms of complexity), view synthesis in the network has been introduced  for cloud networks \cite{Wen:J13,Melodia:J13}. The desired view is synthesized in the cloud and then sent directly to clients.   However, only the  view requested by the client is synthesized. This means that either the desired view is a priori known  at the source or a switching delay is experienced by the clients.   

In our work, we  propose view synthesis in the network mainly to overcome both uncertainty of users' requests and limited network resources.  In particular, each network node can decide if sending camera views or synthesized (rendered) viewpoints as reference views to neighboring nodes. Other works in the literature have considered reference view optimization for efficient coding \cite{Merkle:J07, DeAbreu:L13} and streaming strategies \cite{ren15, DeAbreu:C14}. However, reference view selection was limited to camera views. 
  





 
 

==> results_old.tex <==
\begin{table*}[t]
\begin{center}
\caption{Viewpoints notation. } \label{table:views_notation}
\begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|c|c|} \hline 
Camera ID as in \cite{Kim:SRLF:2013}, ``Statue" & $ {50}$ & $51$  & $52$ & $53$ & $54$ & $55$ & $56$ & $57$ & $ {58}$ & $59$ & $\ldots$ & $ {98}$      \\ \hline
Camera ID as in \cite{Kim:SRLF:2013}, ``Mansion" & $ {25}$ & $26$  & $27$ & $28$ & $29$ & $30$ & $31$ & $32$ & $ {33}$ & $34$ & $\ldots$ & $ {73}$      \\ \hline\hline
Camera ID in our work & $ {0}$ & $1.125$  & $1.25$ & $1.375$ & $1.5$ & $1.625$ & $1.75$ & $1.875$ & $ {1}$ & $2.125$ & $\ldots$ & $ {6}$    \\ \hline 
\end{tabular}
\end{center}
\end{table*}
 
%%%%%%%%%%% 
\subsection{Settings}
We study the performance of our algorithm and we show the distortion gains due to the view  synthesis in the network. For a given range of interest $[U_L^0,U_R^0]$, we provide the average quality (evaluated as the PSNR of the average distortion)  at which any viewpoint in the range is synthesized. This means that the average distortion of the range is evaluated as $(1/N)\sum_{u=U_L^0}^{U_R^0} d_u$, with $N$ being the number of synthesized viewpoints in the range of interest.  Finally, for the sake of clarity, in the following we denote by $\mathcal{T}_{s}$ the subset of selected reference views when synthesis is allowed in the network, and by 
$\mathcal{T}_{ns}$ the subset of selected reference views when only camera views can be sent as reference views, i.e., when synthesis is not allowed in the network. 

The   results have been carried out using   3D sequences   
 where $51$ cameras acquire the scene with uniform spacing between the camera positions. The spacing between camera positions is $5.33$ mm and $10$ mm for the ``Statue" and ``Mansion" sequences~\cite{Kim:SRLF:2013}, respectively. Finally, among all camera views provided for both sequences, we consider only a subset available at the edge server, i.e.,  in $\mathcal{V}$, while the remaining   have to be synthesized.   Table \ref{table:views_notation} depicts how the camera  notation used in \cite{Kim:SRLF:2013}   is adapted to our notation.  
For both the cases of network synthesis and no network  synthesis, the best subset of reference views is evaluated both with the proposed  view selection algorithm   with an exact solution, i.e., an exhaustive search of all possible combinations of reference views. For the proposed algorithm, the distortion is evaluated both with  experimental computation of the distortion, where the  results are labeled ``Proposed Alg. (Experimental Dist)",  and with the   model in     \eqref{eq:distortion_model}, results labeled ``Proposed Alg. (Theoretical Dist)".  
For all three   algorithms, once the optimal subset of reference view is selected,  the full range is reconstructed experimentally and the mean PSNR of the actual reconstructed sequence is computed.


 
In our algorithm, we have considered the following  model for the distortion of the synthesized viewpoint $u$ from   reference views $V_L$, $V_R$  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
\label{eq:distortion_model}
 d_u (V_L, V_R, D_L, D_R)  = \alpha D_{min} + (1-\alpha) \beta D_{max} + 
\left[ 1-  \alpha  -  (1-\alpha) \beta \right] D_{I}
\end{align}
where $D_{min}=\min\{D_L,D_R\}$, $D_{max}=\max\{D_L,D_R\}$, $D_I$ is the inpainted distortion, and 
$ 
 \alpha = \exp\left(-\gamma |u-V_{min}| d\right), \,
 \beta = \exp\left(-\gamma |u-V_{max}| d\right) \nonumber
$ 
with  $d$ is the distance between two consecutive camera views $v_i$ and $v_{i}+1$,    $V_{min}=V_L$ if $D_L\leq D_R$, $V_{min}=V_R$ otherwise, and $V_{max}=V_L$ if $D_L>D_R$, $V_{max}=V_R$. 
The model can be explained as follows. A virtual synthesis $u$, when reconstructed from $(V_L,V_R)$ has a relative portion $\alpha\in[0,1]$ that is reconstructed  at a distortion $D_{min}$, from the dominant reference view, defined as the one with minimum distortion. The remaining portion of the image, i.e., $1-\alpha$, is either reconstructed by the non-dominant reference view for a potion  $\beta$, at a distortion $D_{max}$, or it is inpainted, at a  distortion $D_I$.

In the following,   we first validate the above distortion model and  the optimization algorithm and the distortion model. Then, we provide simulation using the model in   \eqref{eq:distortion_model} and study the gain offered by network synthesis.



  
  
 
\begin{figure}[t]
\subfigure[Mansion]
{\label{fig:Mansion_validation_equallySpaced}
\includegraphics[width=0.48\linewidth ,draft=false]{figure/Mansion_validation_equallySpaced.eps}  
}  \hfill   
%%%
\subfigure[Statue]{\label{fig:Statue_validation_equallySpaced}
\includegraphics[width=0.48\linewidth ,draft=false]{figure/Statue_validation_equallySpaced.eps}
}   \caption{Validation of the proposed optimization model  in the setting of  an equally spaced cameras set  $\mathcal{V}=\{0,1, 2, \ldots, 5, 6\}$, and range of interest of  $[0.75,5.25]$. (a) ``Mansion"  sequence, for  the theoretical model, $\beta=0.2$, $D_{max}=450$, $d=50$. (b) ``Statue" sequence,   for the theoretical model, $\beta=0.2$, $D_{max}=100$, and $d=25$mm.  } \label{fig:Statue_Validation}
\end{figure}

%
%\begin{figure}[t]
%\begin{center}
%\includegraphics[width=0.65\linewidth ,draft=false]{figure/Mansion_validation_equallySpaced.eps} 
%\caption{Validation of the proposed optimization model for ``Mansion" sequence in the setting of  an equally spaced cameras set  $\mathcal{V}=\{0,1, 2, \ldots, 5, 6\}$, and range of interest of  $[0.75,5.25]$. For }\label{fig:Mansion_validation_equallySpaced}
%\end{center}
%\end{figure}

 
%\begin{figure}
%\subfigure[Equally spaced cameras, $\mathcal{V}=\{0,1, 2, 3, 4, 5, 6\}$.]
%{\label{fig:Statue_validation_equallySpaced}
%\includegraphics[width=0.48\linewidth ,draft=false]{figure/Statue_validation_equallySpaced.eps}  
%}  \hfill   
%%%
%\subfigure[Unequally spaced cameras, $\mathcal{V}=\{0,1.5, 2, 2.75, 4, 5, 6\}$.]{\label{fig:Statue_Validation_Unequally}
%\includegraphics[width=0.48\linewidth ,draft=false]{figure/Statue_Validation_Unequally.eps}
%}   \caption{Validation of the proposed optimization model for ``Statue" sequence for a range of interest of  $[0.75,5.25]$. For the theoretical model, $\beta=0.2$, $D_{max}=100$, and $d=25$mm. Red curves provide results when synthesis is allowed in the network. Blue curves provide results when synthesis is  not allowed in the network.} \label{fig:Statue_Validation}
%\end{figure}



%%%%%%%%%%%%
\subsection{Performance of the view selection algorithm}
In Fig. \ref{fig:Mansion_validation_equallySpaced}, we provide the mean PSNR as a function of the available bandwidth $C$ for the ``Mansion"  sequence in the setting of  a regular spaced cameras set  $\mathcal{V}=\{0,1, 2, \ldots, 5, 6\}$, and range of interest of views in   $[0.75,5.25]$ for the user. For the theoretical distortion model, we used $\beta=0.2$, $D_{max}=450$, and $d=50$. The proposed algorithm with experimental distortion perfectly matches the exhaustive search. Also the proposed algorithm based on theoretical distortion nicely matches the exhaustive search method, with the exception of $C=4$ and synthesis allowed. In this case, the algorithm selects as best subset $\mathcal{T}_s=\{ 0.75, 2, 4, 5.25\}$ rather than $\mathcal{T}_{ns}=\{ 0.75, 2, 3, 5.25\}$. 
Beyond the good match between exhaustive search and proposed algorithm, Fig. \ref{fig:Mansion_validation_equallySpaced} also shows the gain achieved in synthesizing reference views. In particular, the possibility of selecting $0.75$ as reference view leads to save bandwidth since one view can be sent, rather than sending two camera views, namely  $0$ and $1$. At the same time, only camera view $0$ could be sent, but this would increase the distance between the reference view and any viewpoint in the range of interest $[0.75,5.25]$. Thus, as long as the viewpoint $0.75$ is synthesized at a good quality and the channel bandwidth  $C$ is limited, synthesizing in the network improved the quality of the reconstructed region of interest. 

Similar considerations can be derived from Fig. \ref{fig:Statue_validation_equallySpaced}, where the same setting of before is considered but for the ``Statue"  sequence. Also in this case we observe a very good match between the proposed algorithm and the exhaustive search one. 

\begin{figure}
\begin{center}
\includegraphics[width=0.48\linewidth ,draft=false]{figure/Statue_Validation_Unequally.eps}
  \caption{Validation of the proposed optimization model for ``Statue" sequence in the settings of unequally spaces cameras $\mathcal{V}=\{0,1.5, 2, 2.75, 4, 5, 6\}$ and  range of interest of  $[0.75,5.25]$. For the theoretical model, $\beta=0.2$, $D_{max}=100$, and $d=25$mm. Red curves provide results when synthesis is allowed in the network. Blue curves provide results when synthesis is  not allowed in the network.} \label{fig:Statue_Validation}
\end{center}
\end{figure}


Finally, in Fig. \ref{fig:Statue_Validation_Unequally}, we compare the exhaustive search algorithm with our optimization method in the case of non-equally spaced cameras. The ``Statue" sequence is considered in the setting of     unequally spaced cameras set  $\mathcal{V}=\{0,1.5, 2, 2.75, 4, 5, 6\}$, and range of interest of  $[0.75,5.25]$. For the theoretical model, $\beta=0.2$, $D_{max}=100$, and $d=25$mm.  
Similarly to the equally spaced scenario, the proposed optimization matches the exhaustive search. Also, a quality gain is experienced in selecting synthesized viewpoints as reference views (red curves) with respect to the case of only camera view selection. The maximum gain is achieved for $C=2$, with $\mathcal{T}_s=\{0.75,5.25\}$ and $\mathcal{T}_{ns}=\{0,6\}$. Increasing the channel capacity, camera views are selected as inner reference views, as the case of  $C=3$, with $\mathcal{T}_s=\{0.75, 2.75, 5.25\}$ and $\mathcal{T}_{ns}=\{0, 2.75, 6\}$. 


 
\subsection{Gain in Synthesizing in the Network}
%We now provide further results  to show when it is worthy to select virtual viewpoints as reference views. 
    We now study  the quality performance behavior when synthesis is allowed in the network for different synthetic scenarios. We adopt the distortion model in   \eqref{eq:distortion_model} for both solving the optimization algorithm and evaluating the system performance. % with $\gamma=0.2$, $D_I=200$, and $d= 25\text{mm}$ for most of the following results. 
%\footnote{Note that we have simulated many different scenarios (i.e., different parameters in the distortion model). Since   very similar results have been experienced, here we do not provide the entire simulated settings. } 
%Simulation results are provided for both the case in which synthesis is allowed in the network and the one in which only camera views can be selected as reference views. The main goal is to show under which circumstances  it is worthy to select virtual viewpoints as reference views.  
%\begin{figure}[t]
%\begin{center}
%\subfigure[Equally spaced cameras with $\mathcal{V}=\{0,1,2, \ldots, 8\}$]{\label{fig:Camera_Setting_A}
%\includegraphics[width=0.48\linewidth ,draft=false]{figure/Camera_Setting_A.eps}
%} \hfill
%\subfigure[Unequally spaced cameras with  $\mathcal{V}=\{0, 1, 3, 5, 7, 8\}$]{\label{fig:Camera_Setting_B}
%\includegraphics[width=0.48\linewidth ,draft=false]{figure/Camera_Setting_B.eps}
%} \hfill
%\subfigure[Unequally spaced cameras with  $\mathcal{V}=\{0, 2, 3, 4, 7, 8\}$]{\label{fig:Camera_Setting_C}
%\includegraphics[width=0.48\linewidth ,draft=false]{figure/Camera_Setting_C.eps}
%} \hfill
%\caption{Different camera settings considered in the simulation results for a range of interest $[0.75,7.25]$. }\label{fig:Camera_Setting}
%\end{center}
%\end{figure}
We consider both cases of equally  spaced cameras $\left(\mathcal{V}=\{0,1, 2, \ldots, 5, 6\}\right)$  and unequally spaced cameras $\left(\mathcal{V}=\{0, 1, 3,  5, 7,  8\}\right.$  and  $\left.\mathcal{V}=\{0, 2, 3, 4, 7, 8\}\right)$  capturing the scene of interest.  %is depicted in Fig. \ref{fig:Camera_Setting_A}, where 
%%each camera is spaced of a distance $d$ between each other and the entire camera set is . To simulate the unequally spaced camera setting, we consider two different camera sets 
%% $\mathcal{V}=\{0, 1, 3,  5, 7,  8\} $ and $\mathcal{V}=\{0, 2, 3, 4, 7, 8\}$.%, respectively Fig. \ref{fig:Camera_Setting_B}  and  Fig. \ref{fig:Camera_Setting_C}.
%A non-uniform sampling of the camera set  leads to unequally spaced camera settings.
 Note that the distance between two camera views $v_j$ and $v_i$ is evaluated as $|v_j-v_i| d$, for example $2d$ is the distance between view $0$ and view $2$.  In  the case of equally spaced cameras, each camera is spaced of a distance $d$ between each other. %\note{Do you think that we have to put the Fig. 6 or could we simply rely on the word-description of the set? Also, we could delete Fig. 7 (equal spaced case) if we need room. }


\begin{figure}
  \begin{minipage}[c]{0.50\linewidth}
    \centering
\includegraphics[width=1\linewidth ,draft=false]{figure/PSNR_vs_C.eps} 
  \end{minipage}
  \begin{minipage}[c]{0.50\linewidth}
    \centering
%\caption{Selected subset of reference views and associated quality for scenarios with $[U_L^0,U_R^0]=[0.75,7.25]$ , $\mathcal{V}=\{0, 1, 2, 3, 4, 5, 6\}$, case $a)$ of Fig. \ref{fig:Camera_Setting},  $\gamma=0.2$, $D_{max}= 300$. } \label{table:Selected_Views_EqSpaced}
  %  \vspace{-3cm} \
\begin{tabular}{|c||c||c|c|c|c|c|c|c|c|c|c|} \hline 
$C $ & $\mathcal{T}_{s}$ &      $\mathcal{T}_{ns}$        \\ \hline\hline
$2$  & $\{0.75, 5.25\}$ &     $\{\pmb{0}, \pmb{6}\}$       \\ \hline
$3$  & $\{0.75, \pmb{3},  5.25\}$ &       $\{\pmb{0}, \pmb{3}, \pmb{6}\}$       \\ \hline
$4$  & $\{0.75, \pmb{2}, \pmb{4}, 5.25\}$  &     $\{\pmb{0}, \pmb{2}, \pmb{4}, \pmb{6}\}$       \\ \hline
$5$  & $\{0.75, \pmb{2}, \pmb{3}, \pmb{4}, 5.25\}$ &   $\{\pmb{0}, \pmb{2}, \pmb{3}, \pmb{4}, \pmb{6}\}$      \\ \hline
$6$  & $\{ \pmb{0},  \pmb{1},  \pmb{2}, \pmb{3}, \pmb{4}, 5.25\}$ &    $\{\pmb{0}, \pmb{1}, \pmb{2}, \pmb{3}, \pmb{4}, \pmb{6}\}$     \\ \hline
$7$  & $\{ \pmb{0},  \pmb{1}, \pmb{2}, \pmb{3}, \pmb{4}, \pmb{5}, \pmb{6}\}$ &      $\{\pmb{0}, \pmb{1}, \pmb{2}, \pmb{3}, \pmb{4}, \pmb{5}, \pmb{6}\}$      \\ \hline
  \end{tabular}
  \par\vspace{0pt}
\end{minipage}
\caption{Mean quality and optimal subsets  for different channel capacity values  $C$ for a regular spaced camera set with varying distance among cameras, $\gamma=0.3$, $D_I=300$,  range of interest $[0.75,5.25]$, and camera set $\mathcal{V}=\{0,1, 2, \ldots, 5, 6\}$ (equally spaced cameras). On the left, curves showing the PSNR behavior as function of the channel capacity $C$. On the right, the table shows the optimal subsets for each channel capacity $C$. }\label{fig:PSNR_vs_C_varying_d}
\end{figure}

%\begin{figure}[t]
%\begin{center}
%\includegraphics[width=0.75\linewidth ,draft=false]{figure/PSNR_vs_C_varying_d_3.eps} 
%\caption{PSNR vs. $C$ for a regular spaced camera set with varying distance among cameras, $\gamma=0.3$, $D_I=300$,  range of interest $[0.75,5.25]$, and camera set $\mathcal{V}=\{0,1, 2, \ldots, 5, 6\}$ (equally spaced cameras).}\label{fig:PSNR_vs_C_varying_d}
%\end{center}
%\end{figure}
 %\begin{table*}[t]
%\begin{center}
%\caption{Selected subset of reference views and associated quality for scenarios with $[U_L^0,U_R^0]=[0.75,7.25]$ , $\mathcal{V}=\{0, 1, 2, 3, 4, 5, 6\}$, case $a)$ of Fig. \ref{fig:Camera_Setting},  $\gamma=0.2$, $D_{max}= 300$. } \label{table:Selected_Views_EqSpaced}
%\begin{tabular}{|c||c||c|c|c|c|c|c|c|c|c|c|} \hline 
%$C $ & $\mathcal{T}_{s}$ &      $\mathcal{T}_{ns}$        \\ \hline\hline
%$2$  & $\{0.75, 5.25\}$ &     $\{\pmb{0}, \pmb{6}\}$       \\ \hline
%$3$  & $\{0.75, \pmb{3},  5.25\}$ &       $\{\pmb{0}, \pmb{3}, \pmb{6}\}$       \\ \hline
%$4$  & $\{0.75, \pmb{2}, \pmb{4}, 5.25\}$  &     $\{\pmb{0}, \pmb{2}, \pmb{4}, \pmb{6}\}$       \\ \hline
%$5$  & $\{0.75, \pmb{2}, \pmb{3}, \pmb{4}, 5.25\}$ &   $\{\pmb{0}, \pmb{2}, \pmb{3}, \pmb{4}, \pmb{6}\}$      \\ \hline
%$6$  & $\{ \pmb{0},  \pmb{1},  \pmb{2}, \pmb{3}, \pmb{4}, 5.25\}$ &    $\{\pmb{0}, \pmb{1}, \pmb{2}, \pmb{3}, \pmb{4}, \pmb{6}\}$     \\ \hline
%$7$  & $\{ \pmb{0},  \pmb{1}, \pmb{2}, \pmb{3}, \pmb{4}, \pmb{5}, \pmb{6}\}$ &      $\{\pmb{0}, \pmb{1}, \pmb{2}, \pmb{3}, \pmb{4}, \pmb{5}, \pmb{6}\}$      \\ \hline
%  \end{tabular}
%\end{center}
%\end{table*}
\begin{table*}[t]
\begin{center}
\caption{Selected subset of reference views and associated quality for scenarios with $[U_L^0,U_R^0]=[0.75,7.25]$ , $d=25$ mm, $\gamma=0.2$, $D_{max}= 200$. } \label{table:Selected_Views_NonEqSpaced}
\begin{tabular}{|c||c|c||c|c|c|c|c|c|c|c|c|c|} \hline 
\multicolumn{5}{|c|}{$\mathcal{V}=\{0, 1, 3,  5, 7,  8\} $, case $a)$  } \\ \hline
$C $ & $\mathcal{T}_{s}$ &  PSNR &    $\mathcal{T}_{ns}$ &  PSNR         \\ \hline\hline
$2$  & $\{0.75, 7.25\}$ &  29.39 &   $\{\pmb{0}, \pmb{8}\}$  &    28.04 \\ \hline
$3$  & $\{0.75, \pmb{3}, 7.25\}$ &  32.35  &  $\{\pmb{0}, \pmb{3}, \pmb{8}\}$  &  31.13  \\ \hline
$4$  & $\{0.75, \pmb{3}, \pmb{5}, 7.25\}$ &  35.24 &  $\{\pmb{0}, \pmb{3}, \pmb{5}, \pmb{8}\}$   &   33.87 \\ \hline
$5$  & $\{\pmb{0}, \pmb{1},  \pmb{3}, \pmb{5}, 7.25\}$ &  35.85  &   $\{\pmb{0}, \pmb{1},  \pmb{3}, \pmb{5}, \pmb{8}\}$  &  35.017 \\ \hline
$6$  & $\{\pmb{0}, \pmb{1},  \pmb{3}, \pmb{5}, \pmb{7}, \pmb{8} \}$ &   36.56 &  $\{\pmb{0}, \pmb{8}\}$   &  36.56
  \\ \hline\hline
  %%%%%%%%%%%%%%%%
\multicolumn{5}{|c|}{$\mathcal{V}=\{0, 2, 3, 4, 7, 8\}$, case $b)$ } \\ \hline
$C$  & $\mathcal{T}_{s}$ &  PSNR    & $\mathcal{T}_{ns}$ &  PSNR       \\ \hline\hline
 $2$ &  $\{0.75, 7.25\}$ & 29.08  &     $\{\pmb{0}, \pmb{8}\}$     &  28.04   \\ \hline
 $3$ &  $\{0.75, \pmb{4}, 7.25\}$ &  32.33  &    $\{ \pmb{0},   \pmb{4},  \pmb{8} \}$ &   31.49  \\ \hline
$4$ &  $\{\pmb{0},  \pmb{2},  \pmb{4}, 7.25\}$ &  34.18 &  $\{ \pmb{0}, \pmb{2}, \pmb{4},  \pmb{8}\}$ &  33.21   \\ \hline
$5$ &  $\{\pmb{0},  \pmb{2},  \pmb{4}, \pmb{7}, \pmb{8}\}$ &    34.92 & $\{ \pmb{0}, \pmb{2}, \pmb{4}, \pmb{7}, \pmb{8} \}$ &    34.92     \\ \hline
$6$ &  $\{\pmb{0},  \pmb{2},  \pmb{3}, \pmb{4}, \pmb{7}, \pmb{8}\}$ &    35.60 & $\{ \pmb{0}, \pmb{2}, \pmb{4}, \pmb{7}, \pmb{8} \}$ &    35.60     \\ \hline
  \end{tabular}
\end{center}
\end{table*}

 In Fig. \ref{fig:PSNR_vs_C_varying_d}, we show the mean PSNR as a function of the available channel capacity $C$ when the range of interest is $[0.75,5.25]$ and the set of equally spaced cameras   $\mathcal{V}=\{0,1, 2, \ldots, 5, 6\}$.   The distortion of synthesized viewpoints is evaluated from  \eqref{eq:distortion_model}, with $\gamma=0.2$, $D_I=200$, and $d= 25\text{mm}$. % We recall that in this subsection we theoretically evaluate  the distortion function from  Eq.  \eqref{eq:distortion_model} both for solving the optimization algorithm and for evaluating the average quality of the reconstructed range of interest.  
    The case of synthesis in the network is compared with the one in which only camera views can be sent to clients. In Fig. \ref{fig:PSNR_vs_C_varying_d}, for each PSNR value provided on the left, we show the associated optimal subset $\mathcal{T}_s$ or $\mathcal{T}_{ns}$ in the table on the right. In the table,   camera views indexes are highlighted in bold.
We observe that   the case of synthesis in the network performs best in terms of quality of the reconstructed viewpoints range.   When $C=2$, $\mathcal{T}_{s}:\{0.75,5.25\}$ for the synthesis allowed case, and $\mathcal{T}_{ns}:\{0, 6\}$, otherwise. When the channel capacity increases and synthesis is allowed in the network,  the lateral  reference views are still $0.75$ and $5.25$ while the inner ones are camera views. For example, for $C=4$, $\mathcal{T}_{s}:\{0.75, 2, 4, 5.25\}$ and $\mathcal{T}_{ns}:\{0, 2, 4, 6\}$. However, the larger the channel capacity the less the need for sending virtual viewpoints. When $C=6$, for example, both camera views $0$ and $1$ can be sending, thus there is no gain in transmitting to clients only $0.75$, which is synthesized from the camera views $0$ and $1$.  Finally,  when $C=7$ and all camera views can be sent to clients, $\mathcal{T}_{s} = \mathcal{T}_{ns} =\mathcal{V}$, with   $\mathcal{V}$ being the set of camera views. Thus, sending synthesized viewpoints as reference views leads to a quality gain only in constrained scenarios in which the channel capacity does not allow to send all views required for reconstructed the range of interest. 
 


\begin{figure}[t]
\begin{center}
\includegraphics[width=0.65\linewidth ,draft=false]{figure/PSNR_vs_DeltaU.eps} 
\caption{PSNR vs. $U_L^0$ for a  camera set $\mathcal{V}=\{0, 2, 3, 4\}$, range  of interest $[U_L^0, 4]$, with  $d=50$mm, $\gamma=0.2$, and $D_I=200$.}\label{fig:PSNR_vs_DeltaU}
\end{center}
\end{figure}

We now study the gain in allowing synthesis in the network when camera views are not-equally spaced.  In Table \ref{table:Selected_Views_NonEqSpaced}, we provide  the optimal subsets of reference views for both cases of unequally spaced cameras $\left(\mathcal{V}=\{0, 1, 3,  5, 7,  8\}\right.$  and  $\left.\mathcal{V}=\{0, 2, 3, 4, 7, 8\}\right)$.  Similarly to the case of equally spaced cameras, we observe that virtual viewpoints are selected as reference views (i.e., they are in the best subset $\mathcal{T}_s$) only   at the extreme of the range of interest. Moreover,  in the scenario $a)$, for $C=4$ the view $0.75$ is selected as reference view, while the scenario      $b)$  prefers to select the camera views $0$, $2$. This is justified by the fact that in the latter scenario, the viewpoint $0.75$ is synthesized from $(V_L,V_R)=(0,2)$ thus at a larger distortion than the viewpoint $0.75$ in   scenario  $a)$, where the viewpoint is synthesized from $(V_L,V_R)=(0,1)$. This penalty in distortion makes the synthesis worthy when the channel bandwidth is highly constrained ($C=2, 3$), but not in the rest of the cases. 
 
   

 


 In Fig. \ref{fig:PSNR_vs_DeltaU}, the average quality is provided as a function of the left extreme of the range of interest, i.e., $U_L^0$ for a scenario with camera set $\mathcal{V}=\{0, 2, 3, 4\}$, range  of interest $[U_L^0, 4]$, with  $d=50$mm, $\gamma=0.2$, and $D_I=200$. It is worth noting that $U_L^0$ ranges from $0$ to $1.875$ and only view  $0$ is   a camera view in this range.   When $U_L^0=0$ and $C=2$, the reference views $0$ and $4$ perfectly covers the entire range of interest, so there is no need of sending any  virtual viewpoint as reference view. This is no more true   for $U_L^0>0$. When the channel capacity is $C=2$, the gain in allowing synthesis at the source increases with   $U_L^0$. This is justified by the fact that in a very challenging scenario (i.e., limited channel capacity), the larger is $U_L^0$ the less efficient is sending the reference view $0$ to reconstruct the range $[U_L^0,4]$. At the same time, sending $2$ and $4$ as reference views would not allow to reconstrcut   the viewpoints lower than $2$. This gain in synthesizing is reflected in the PSNR curves of Fig.  \ref{fig:PSNR_vs_DeltaU}, where we can observe that for $C=2$ there is an increasing gap between the case of synthesis allowed and not allowed. This gap is however reduced for the scenario of $C=3$. This is expected since the range of interest under consideration is a limited one, at most ranging from $0$ to $4$ and   $4$ reference views would already perfectly recover the range. %%%%\blue{Thus, for the scenario of interest,  $C=3$ is not a highly challenging case. In particular, for all $U_L^0$ ranging from $0$ to $1.625$, it is worthy to send both camera views $0$ and $2$ rather than a synthesized reference view in the middle.  Note that sending a virtual viewpoint equal to $U_L^0$ rather than the couple $(0, 2)$ as reference view would lead to bandwidth gain that can then be used to send camera view $3$ beyond camera view $4$. While when $(0, 2)$ are sent, the camera view $3$ is scarified and not sent to clients. However, since the quality of the synthesized viewpoint $U_L^0$ is not the minimum one (since it is reconstructed from $0$ and $2$ rather than from $0$ and $1$), the bandwidth gain has a price to pay (increasing distortion of the reference view) which is not worthy to be paid. This confirms the behavior already observed before which is that a virtual viewpoint is selected as reference view only in scenarios with highly limited network resources. }
       

%%%%DECOMMENT TO SEE THE EXTRA FIGURE
%\begin{figure}[t]
%\begin{center}
%\includegraphics[width=0.75\linewidth ,draft=false]{figure/BestC_vs_UR.eps} 
%\caption{Thresholding $C$ vs. $U_R^0$  for a range of interest of $[0.5, U_R^0]$, with  $d=50$mm, $\gamma=0.2$, and $D_I=200$.}\label{fig:BestC_vs_UR}
%\end{center}
%\end{figure}
%To better show this tradeoff between distortion of the virtual reference view and  the bandwidth gain, 
%we introduce the  thresholding channel value, denoted by $C^{\star}$. The latter is defined as the value of channel bandwidth beyond which no gain is experienced in allowing synthesis in the network compared to a case of no synthesis. In Fig. \ref{fig:BestC_vs_UR}, we provide the behavior of the thresholding channel value as a function range of interest, for different cameras set. In particular, we consider $U_L^0=0.5$ and we let $U_R^0$ varies from $5$ to $10$. Also, we simulate three different scenarios that differ for the available camera set. In particular, we have $\mathcal{V}= \{0,1, 2, 3, \ldots\}$, $\mathcal{V}= \{0, 2, 3, 4, \ldots\}$, and $\mathcal{V}= \{0, 3, 4, 5,  \ldots\}$. The main difference is then in the reference views that can be used to synthesize the virtual viewpoint $0.5$. In the first case, $0.5$ is reconstructed from camera views $(0,1)$ while in the last case from $(0,3)$ increasing then the distortion of the synthesis. Because of this increased distortion of $0.5$, the virtual viewpoint is not always sent as reference view. In particular, we can observe that the larger the distortion of the virtual viewpoint, the lower the thresholding channel value. This means that even in challenging scenarios, as for example in the case of $U_R^0=7$ and $C=3$, if $\mathcal{V}= \{0, 3, 4, 5,  \ldots\}$ 
% then there is no gain in synthesize in the network, while we still have a gain if $\mathcal{V}= \{0,1, 2, 3, \ldots\}$.

 
 

 \begin{figure}[t]
\begin{center}
\includegraphics[width=0.65\linewidth ,draft=false]{figure/DeltaPSNR_vs_RangeInterest.eps} 
\caption{ PSNR gain (in dB) vs. the range of interest size $\Delta_u$, for different channel capacity constraints $C$ when  $d=50$mm, $\gamma=0.2$, and $D_I=200$.}\label{fig:DeltaPSNR_vs_RangeInterest}
\end{center}
\end{figure}


  
In Fig. \ref{fig:DeltaPSNR_vs_RangeInterest},  we provide the mean PSNR as a function of the size of the range of interest, namely $\Delta_u$. More in details, for each value of $\Delta_u$, we define the range of interest as $[U_L^0, U_L^0+ \Delta_u]$. The starting viewpoint $U_L^0$ is randomly selected. For each realization of the range of interest, the best subset is evaluated (both when synthesis is allowed and when it is not) and the quality of the reconstructed viewpoint range is evaluated. For each  $\Delta_u$, we average the quality simulating all possible $U_L^0$ starting viewpoint within a total range of $[0,12]$. In the results we provide the PSNR gain, defined as the difference between the mean PSNR (in dB) when the synthesis is allowed and the  mean PSNR (in dB) when only  camera views are considered as reference views. Thus, the figure shows the gain in synthesizing for different sizes of the range of interest. As general trend, we observe that the quality gain decreases with  $\Delta_u$. This is due to the fact that the gain mainly comes from the lateral reference views, that are usually virtual viewpoints if synthesis is allowed. This leads to a gain that is however reduced for large sizes of the range of interest. 
Finally, we also observe that the gain does not necessarily depends on the channel constraint $C$.  



\begin{figure}[t]
\begin{center}
\includegraphics[width=0.65\linewidth ,draft=false]{figure/Q_vs_Randomness.eps} 
\caption{ PSNR  (in dB) vs.   $\sigma_v^2$, for different channel capacity constraints $C$ when  $d=50$mm, $\gamma=0.2$, and $D_I=200$.}\label{fig:Q_vs_Randomness}
\end{center}
\end{figure}

We now   consider a scenario in which camera view position is not a priori given. In Fig. \ref{fig:Q_vs_Randomness}, we provide the mean PSNR as a function of the variance $\sigma_v^2$, which defines the randomness in locating the camera views when acquiring the scene. More in details, we consider a range of interest $[U_L^0,U_R^0]=[2,6]$. We then define a deterministic camera views set $\mathcal{V}_D=\{0,1,2, \ldots, 7\}$, which is the best camera view set since it is aligned with the requested viewpoint range. For each value of $\sigma_v^2$, we generate a random cameras set  $\mathcal{V}$ as $\mathcal{V} =\mathcal{V}_D + [n_0, n_1, \ldots, n_7]$, where each $n_i$ is a gaussian random variable with zero mean and variance $\sigma_v^2$ with $n_i$ and $n_j$ mutually independent for $i\neq j$. Thus, the larger $\sigma_v^2$, the larger the probability for the camera view set  to be not aligned with the range of interest. For each $\mathcal{V}$ we run our optimization for both the cases of allowed and not allowed synthesis and we evaluate the experienced quality. For each $\sigma_v^2$ value we simulate $400$ runs and we provide in  Fig. \ref{fig:Q_vs_Randomness} the averaged quality. 
What it is interesting to observe is that even if camera views are not perfectly aligned with the range of interest (i.e., even for large variance values) the quality degradation with respect to the case of $\sigma_v^2=0$ is limited, about $0.5$ dB for $C=3$. On the contrary, when synthesis is not allowed in the network, the quality substantially decreases with $\sigma_v^2$, experiencing a PSNR loss of almost $1.5$dB.  

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.65\linewidth ,draft=false]{figure/Q_vs_Cameras.eps} 
\caption{ PSNR   (in dB) vs. the sampling ditance $S$,  for $C=2$,   $d=50$mm, $\gamma=0.2$, and $D_I=200$.}\label{fig:Q_vs_Cameras}
\end{center}
\end{figure}

Finally, we consider a scenario in which the camera views are equally spaced and the distance between consecutive camera views is a multiple of $d$, with $d=50$mm. Namely, we  consider $S d$ the distance between consecutive cameras, and we provide the quality behavior for $S$ ranging from $1$ to $12$. While the position of camera views changes with $S$, we assume a fixed set of virtual viewpoints $\mathcal{U}$ with consecutive viewpoints at constant distant $d$. This means that when $S=1$, the set of viewpoints $\mathcal{U}$ is equivalent to the camera views set $\mathcal{V}$, while for  $S=2$, every two viewpoints in $\mathcal{U}$ one is a camera view and so on.  
For each value of the sampling distance $S$, we simulate a range of interest spanning a distance of $20 d$. The range of interest is 
randomly selected and the optimization algorithm evaluates the best subset of reference views. The experienced quality is averaged over $400$ runs and evaluated for different values of  $S$.  
In Fig. \ref{fig:Q_vs_Cameras}, we show the mean quality of the reconstructed range as a function of the sampling distance $S$, for the scenario with  for $C=2$,   $d=50$mm, $\gamma=0.2$, and $D_I=200$. When synthesis is allowed,  we   notice the gains in terms of sampling distance, which means a gain in the number of camera views that have to acquire the 3D scene. In particular, to achieve a given quality, say $33$ dB as highlighted in the figure, the system with no synthesis requires a sampling distance $S=5$, despite the $S=10$ required by the case with synthesis. This means that when synthesis is allowed, half of the number of camera views can be used respect to the case in which no synthesis is allowed. 


 

 





